"The Guide Has Your Back": Exploring How Sighted Guides Can Enhance Accessibility in Social Virtual Reality for Blind and Low Vision People

As social VR applications grow in popularity, blind and low vision users encounter continued accessibility barriers. Yet social VR, which enables multiple people to engage in the same virtual space, presents a unique opportunity to allow other people to support a user's access needs. To explore this opportunity, we designed a framework based on physical sighted guidance that enables a guide to support a blind or low vision user with navigation and visual interpretation. A user can virtually hold on to their guide and move with them, while the guide can describe the environment. We studied the use of our framework with 16 blind and low vision participants and found that they had a wide range of preferences. For example, we found that participants wanted to use their guide to support social interactions and establish a human connection with a human-appearing guide. We also highlight opportunities for novel guidance abilities in VR, such as dynamically altering an inaccessible environment. Through this work, we open a novel design space for a versatile approach for making VR fully accessible.

==> figures/request_style.tex <==
\begin{figure}
\includegraphics[width=50pt]{images/communication_style.png}
\caption{\label{fig: Communication Styles Across 16 Participants.} Distribution of Communication Styles Across 16 Participants. The data is normalized so that the percentages of each request type per participant are added together. These percentages total 1600 across all categories. The numbers displayed are rounded percentages to the nearest whole number, so the displayed sum is 1598.}
\end{figure}

==> figures/utterance_tone.tex <==
\begin{figure}
\includegraphics[width=50pt]{images/request_tone.png}
\caption{\label{fig: Distribution of Tone of Requests Across 16 Participants.} Distribution of Tone of Requests Across 16 Participants. The data is normalized so that the percentages of each request type per participant are added together. These percentages total 1600 across all categories. The numbers displayed are rounded percentages to the nearest whole number, and the displayed sum is 1600.}
\end{figure}

==> text/Description.tex <==
Figure 1: Screenshots of the Tutorial and Three Park Environments from Our Prototype.
A series of seven screenshots depicting the virtual tutorial environment and three different virtual parks. Two screenshots show different angles of a park in the morning with a river and bridges labeled Park 1. Free exploration. Two more show a park at sunset with trees and picnic tables labeled Park 2. Scavenger hunt. The last two show a park in the early afternoon with stone paths and grassy areas labeled Park 3. Free exploration with flying guide.

Figure 2: Likert Scale Responses Histogram
A Likert scale responses histogram showing three statements: 1. I was comfortable with using the guide in this social space; 2. The communication was effective with the guide; 3. The guide was useful. Responses fall mostly in strongly agree (5) for each question, with the next highest amount being agree (4). There is one outlier who put strongly disagree (1) for communication.

Figure 3a: Request Styles Across 16 Participants.
Horizontal bar chart with the x-axis showing the number of requests as the percentage of total requests for each participant ranging from 0 to 800. The y-axis shows 7 different types of request styles. Some examples include “short and simple request,” “open-ended question,” and “request guide to complete an action.” “Short and simple requests” have the highest number with 799. “Multiple choice question” has the smallest with 9.

Figure 3b: Utterance Tone Across 16 Participants.
Horizontal bar chart showing the number of utterances as percentages of the total utterances of each participant ranging from 0 to 1500 on the x-axis. The y-axis shows 5 different utterance tones, including “utilitarian”, “friendly”, and “uncertain.” Five bars are shown. “Utilitarian” is the most common tone with 1358 requests. The least common tone is “uncertain” with 13 utterances.

Table 1: Participants’ Demographics Information
A table depicting participant demographic information for 16 participants, given pseudonyms. Columns from left to right are: pseudonym, age, gender, vision, onset, visual acuity, visual field, and mobility aids.

